The Plot Thickens: Quantitative Part-by-Part Exploration of MLLM Visualization Literacy

Multimodal Large Language Models (MLLMs) can interpret data visualizations, but what makes a visualization understandable to these models? Do factors like color, shape, and text influence legibility, and how does this compare to human perception? In this paper, we build on prior work to systematically assess which visualization characteristics impact MLLM interpretability. We expanded the Visualization Literacy Assessment Test (VLAT) test set from 12 to 380 visualizations by varying plot types, colors, and titles. This allowed us to statistically analyze how these features affect model performance. Our findings suggest that while color palettes have no significant impact on accuracy, plot types and the type of title significantly affect MLLM performance. We observe similar trends for model omissions. Based on these insights, we look into which plot types are beneficial for MLLMs in different tasks and propose visualization design principles that enhance MLLM readability. Additionally, we make the extended VLAT test set, VLAT ex, publicly available on https://osf.io/ermwx/ together with our supplemental material for future model testing and evaluation.

==> content/old_not_used_results.tex <==
\section{Results}

In this section, we present the results of running the MLLMs through our extended VLAT dataset.
We start looking into accuracy and consistency statistics of the MLLMs when all factors but one are held constant.
We then analyze the models' omission rate, run statistics on the effect of plot transformations, and lastly we look into statistical modeling of which visual elements seem to have more impact on the MLLMs' accuracy and omission rates.

\subsection{Accuracy statistics}

We start by looking into some statistics regarding the accuracy of the models with our results dataset grouped and summarized by plot types, underlying datasets, color palettes, types of title, and types of questions.
First, we look into the statistics by plot type, shown in Figure \ref{fig:my_image}.

\begin{figure}[htbp] % h=here, t=top, b=bottom, p=page
    \centering
    \hfill
    \includegraphics[width=0.5\textwidth]{figures/plot_type_hists2} 
    \hfill
    \caption{Distribution of Correct Counts through Plot types}
    \label{fig:acc_plt_type} % Optional label for referencing
\end{figure}

As seen in the figure, Line, Scatter and Bar plots had a very similar results profile.
The distribution of their question results tends towards a bimodal, with 20 and 0 correct being the most common values, while scores in between were much rarer.
Their mean and median are also highly similar: Line had a mean of 10.6 correct answers, and a median of 13.
Scatter had 11.5 mean and 16 median and Bar had a mean of  11.1 and 14 median of correct answers.
Lastly, their standard deviations were also quite similar, being relatively high in all of them: Line had a standard deviation of 8.9, Scatter had 8.8 and Bar had 8.9. Stacked Bar and Percentual Stacked Bar plots, at the other hand, had a completely different profile.
A much higher amount of questions fell on the 0 correct answers bin.
Stacked Bar had slightly better distribution than its Percentual counterpart, having a slightly higher mean and median: Stacked Bar plot type had a mean of 6.91, and median of 3 while the percentual version had 6.11 and median of only 1. 
Their standard deviations were also quite similar at 7.9 and 7.3.
Lastly, the Histogram and the Pie plot type had quite unique results.
The Histogram draws some similarity to the Line, Bar and Scatter plot with a mean of 11.8, a (high) median of 17 and a standard deviation of 8.7.
The Pie plot had the best results among all plot types, with a mean of 18.8, a median of 20, and a standard deviation of only 4 - having the highest mean and median, and lowest standard deviation.

We had rather different results when looking at the same statistics regarding the different color palettes, as seen in Figure~\ref{fig:color_results} below.

\begin{figure}[htbp] % h=here, t=top, b=bottom, p=page
    \centering
    \includegraphics[width=0.5\textwidth]{figures/hist_colors.png} 
    \caption{Distribution of Correct Counts through Color palettes.}
    \label{fig:color_results} % Optional label for referencing
\end{figure}

The different color palettes had almost identical distributions of correct answers.
In all of them, the distribution is highly bimodal, with 20 responses correct being the most common and 0 correct responses being the second most common.
Regarding their means, medians, and standard deviations, three main groups arise.
The slightly more accurate group include Muted Colors and Earthy Tones with means of 10.79 and 10.94, respectively. Their medians are 13 and 14, and their standard deviations 8.82 and 8.23, respectively.
A slightly less accurate group includes Neon Colors, Pastel Colors, Jewel Tones, Cool Tones, Vibrant Colors, Warm Colors and, interestingly, Gray Colors with means ranging from 10.65 to 10.4, medians ranging from 12 to 11, and standard deviations ranging from 8.9 to 8.82.
The negative highlight is the Neutral Colors palette with a mean of 10.06, a median of 10 and a standard deviation of 8.9.

Regarding the last design element that we varied through the plots, Figure~\ref{fig:title_results} shows descriptive statistics and distributions grouped by the types of title.

\begin{figure}[htbp] % h=here, t=top, b=bottom, p=page
    \centering
    \includegraphics[width=0.5\textwidth]{figures/title_hist.png} 
    \caption{Correct count distribution across title types.}
    \label{fig:title_results} % Optional label for referencing
\end{figure}

Noticeably, the distributions are rather similar but the median reveals an interesting finding---later confirmed by the regression analysis.
The plots with a suggestive title have a lower median than the ones with a "normal" title.
Normal titles score a 12 median while suggestive titles end up with 10.


Their mean and median are also highly similar: Line had a mean of 12.77 correct answers, and a median of 18.
Scatter had 11.77 mean and 16 median and Bar had a mean of  
Accuracy statistics by the types of question and by MLLM model have been covered in other works---and interestingly, in  their success rate The models 

\subsection{Omission Statistics}

On top of looking into accuracy statistics, we also look deeper into the distribution, mean, and median of omissions.
As a reminder, every VLAT question (except for one histogram question) includes an \textit{omit} option, allowing the model to abstain from answering.
Here, we analyze omission patterns and statistics based on the design elements we manipulated---namely, plot type, color palette, and title.
First, we look at the distribution of omitted responses across plot types in Figure~\ref{fig:title_ommision}.
In each of the 20 repetitions, the most common value for omissions are 0 and 20.
Once again, plot types Line, Scatter and Bar have similar distributions, but this time for omissions: [put medians and averages]

\begin{figure}[htbp] % h=here, t=top, b=bottom, p=page
    \centering
    \includegraphics[width=0.5\textwidth]{figures/omission1.png} 
    \caption{Omission count distribution over Title Types}
    \label{fig:title_ommision} % Optional label for referencing
\end{figure}

In addition to the plot type breakdown, Figure 8 shows the omission count broken down by combinations of plot type and color palette.

\matheus{Gotta do some sort of correct/omissions}

\gaby{I think it is okay if you do not show all distributions and focus on the most interesting}

\subsection{Transformation statistics}

Apart from looking at the accuracy and omission summary data, the structure of this work allows us to explore the descriptive data of each of the transformations that an original plot went through. To recall, different original plots became new plot types - all plot types they could given their dimensionality. In this small section we quickly look at how shifting from one representation to another payed off, or not.

\begin{figure}[htbp] % h=here, t=top, b=bottom, p=page
    \centering
    \includegraphics[width=0.5\textwidth]{figures/transformation_impact.png} 
    \caption{Title Types' Transformation Impact on Mean Correct Counts}
    \label{In the figure, we average the accuracy of a given plot type in its original form, and compare it with average accuracy in all of the other plot types it was transformed into. Each arrow shows a transformation from an original plot type (departure) to a new plot type (arrival). Every time an arrow is positively inclined, it means that that transformation lead to a higher average accuracy. } % Optional label for referencing
\end{figure}

As we can see from Figure~\ref{fig:my_image}, certain  plot type redefinitions seem really beneficial. Stacked Bar plots being converted into Line Plots, for example, increased the correct counts mean from below 5 to around 10. Pie Charts averaged 20 correct counts once they were turned into simple Bar plots, and Stacked Bar Plots had higher accuracy once turned into their Percentual versions. At the same time, some plot type transformations yield no improve: Bar to Scatter, Line to Bar and Line to Scatter do not strongly alter the accuracy count.

\subsection{Model results}
Most importantly, we are interested in quantifying the effect of different visual elements on the visualization literacy of MLLMs. We explore it in this subsection by looking at their assertion and omission in VLAT questions. To that end, we ran different models described in the last session: two models using normalized correct count as a dependent variable, and two models using normalized omission count as the dependent variable. There are two models for each because in one of them we hold the very dataset as a fixed effect. These results tables follow:

\gaby{The plot type Pie is missing in the table}
\matheus{its not, we need to leave one binary out so that we dont run into problems, the other binaries represent the effect based on that one left out, in this case plot type pie! but i think ill change it to leave a more basic one out} 
\gaby{Ok no worries, then it just needs to be explained in the text}



We also ran different reduced models and residual analysis

\subsection{Residual analysis}
[...]

\subsection{Im using this as an appendix for now}

\begin{table}[htb]
    \caption{\textbf{Plot type impact on MLLM accuracy.}
    3, 2, or 1 stars for significance at 0.1\%, 1\%, and 5\%, respectively.
    The variables under plot types are interactions between a type of question and a plot type: retrieve is short for value retrieval and compare is short for making comparisons.
    Model 1 and 3 were not controlled by datasets, Models 2 and 4 were.}
    \label{tab:model_results-accuracy}
    \centering
    \rowcolors{2}{White}{SteelBlue!20}    
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lllll}
        \toprule
        \textbf{Question and Plot} & \textbf{Model 1} & \textbf{Model 2} & \textbf{Model 3} & \textbf{Model 4}\\
        \toprule
        plot\_type\_hist & \plus0.50 *** & \plus0.27 *** & \plus0.51 *** & \plus0.27 *** \\
        plot\_type\_line & -0.11 ** & \plus0.12 ** & -0.05 & \plus0.18 *** \\
        plot\_type\_pie & \plus0.85 *** & \plus0.14 * & \plus0.86 *** & \plus0.26 ** \\
        plot\_type\_scatter & -0.03 & \plus0.10 ** & -0.04 & \plus0.16 *** \\
        plot\_type\_stacked\_bar & -0.71 *** & -0.46 *** & -0.71 *** & -0.56 *** \\
        plot\_type\_stacked\_bar\_100 & -0.47 *** & -0.31 *** & -0.52 *** & -0.50 *** \\
        retrieve\_hist &  &  & \plus0.18 * & \plus0.19 * \\
        retrieve\_line &  &  & -0.24 *** & -0.24 *** \\
        retrieve\_pie &  &  & \plus0.18 * & \plus0.18 * \\
        retrieve\_scatter &  &  & \plus0.01 & \plus0.01 \\
        retrieve\_stacked\_bar\_100 &  &  & -0.06 & -0.05 \\
        compare\_hist &  &  & \plus0.14 & \plus0.14 \\
        compare\_line &  &  & -0.26 *** & -0.26 *** \\
        compare\_pie &  &  & \plus0.04 & \plus0.04 \\
        compare\_scatter &  &  & -0.09 * & -0.09 * \\
        compare\_stacked\_bar &  &  & -0.08 & -0.08 \\
        compare\_stacked\_bar\_100 &  &  & \plus0.42 *** & \plus0.42 *** \\
        determine\_range\_line &  &  & \plus0.42 *** & \plus0.42 *** \\
        determine\_range\_scatter &  &  & -0.18 *** & -0.18 *** \\
        \bottomrule
    \end{tabular}%
    }
\end{table}


last models

\begin{table}[htb]
    \centering
    \rowcolors{2}{White}{SteelBlue!20}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lrrr}
        \toprule
        \textbf{Variable} & \textbf{Coefficient} & \textbf{p-value} & \textbf{Std. Dev.} \\
        \toprule
        const & 1.07 & 0.00 & 0.09 \\
        openai\_model & 0.28 & 0.00 & 0.04 \\
        referential\_title & 0.04 & 0.31 & 0.04 \\
        dataset\_bar\_data.csv & -1.10 & 0.00 & 0.05 \\
        plot\_type\_pie & -0.04 & 0.57 & 0.06 \\
        plot\_type\_scatter & -0.12 & 0.01 & 0.05 \\
        color\_black & 0.04 & 0.70 & 0.09 \\
        color\_burlywood & 0.06 & 0.51 & 0.09 \\
        color\_chartreuse & 0.03 & 0.71 & 0.09 \\
        color\_lightgray & 0.05 & 0.58 & 0.09 \\
        color\_lightpink & 0.00 & 1.00 & 0.09 \\
        color\_mediumvioletred & -0.02 & 0.82 & 0.09 \\
        color\_red & -0.00 & 0.99 & 0.09 \\
        color\_saddlebrown & 0.01 & 0.96 & 0.09 \\
        color\_tomato & -0.01 & 0.93 & 0.09 \\
        question\_type\_Determine Range & -1.52 & 0.00 & 0.08 \\
        question\_type\_Find Correlations/Trends & -0.00 & 0.90 & 0.00 \\
        question\_type\_Make Comparisons & -1.05 & 0.00 & 0.05 \\
        question\_type\_Retrieve Value & -0.61 & 0.00 & 0.05 \\
        \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{Model 1.}
    Regression results.}
    \label{tab:model1_results}
\end{table}

\begin{table}[htb]
    \centering
    \rowcolors{2}{White}{SteelBlue!20}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lrrr}
        \toprule
        \textbf{Variable} & \textbf{Coefficient} & \textbf{p-value} & \textbf{Std. Dev.} \\
        \toprule
        const & 0.35 & 0.00 & 0.09 \\
        openai\_model & 0.25 & 0.00 & 0.04 \\
        referential\_title & -0.13 & 0.00 & 0.04 \\
        dataset\_line\_data.csv & 0.38 & 0.00 & 0.04 \\
        plot\_type\_bar & -0.02 & 0.65 & 0.05 \\
        plot\_type\_scatter & 0.01 & 0.79 & 0.05 \\
        color\_black & -0.07 & 0.48 & 0.09 \\
        color\_burlywood & 0.06 & 0.55 & 0.09 \\
        color\_chartreuse & -0.00 & 0.96 & 0.09 \\
        color\_lightgray & -0.06 & 0.55 & 0.09 \\
        color\_lightpink & -0.03 & 0.75 & 0.09 \\
        color\_mediumvioletred & -0.01 & 0.92 & 0.09 \\
        color\_red & -0.00 & 0.97 & 0.09 \\
        color\_saddlebrown & 0.07 & 0.49 & 0.09 \\
        color\_tomato & 0.01 & 0.90 & 0.09 \\
        question\_type\_Determine Range & 0.01 & 0.93 & 0.07 \\
        question\_type\_Find Correlations/Trends & -0.27 & 0.00 & 0.07 \\
        question\_type\_Make Comparisons & -1.57 & 0.00 & 0.07 \\
        question\_type\_Retrieve Value & -1.16 & 0.00 & 0.07 \\
        \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{Model 2.}
    Regression results.}
    \label{tab:model2_results}
\end{table}

\begin{table}[htb]
    \centering
    \rowcolors{2}{White}{SteelBlue!20}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lrrr}
        \toprule
        \textbf{Variable} & \textbf{Coefficient} & \textbf{p-value} & \textbf{Std. Dev.} \\
        \toprule
        const & 0.10 & 0.51 & 0.15 \\
        openai\_model & 0.25 & 0.00 & 0.07 \\
        referential\_title & -0.03 & 0.61 & 0.07 \\
        dataset\_stacked\_area\_data.csv & 0.12 & 0.20 & 0.10 \\
        plot\_type\_line & 0.65 & 0.00 & 0.09 \\
        plot\_type\_stacked\_bar\_100 & 0.17 & 0.07 & 0.09 \\
        color\_black & -0.19 & 0.20 & 0.15 \\
        color\_burlywood & -0.07 & 0.63 & 0.15 \\
        color\_chartreuse & -0.01 & 0.94 & 0.15 \\
        color\_lightgray & -0.03 & 0.83 & 0.15 \\
        color\_lightpink & -0.03 & 0.82 & 0.15 \\
        color\_mediumvioletred & -0.04 & 0.80 & 0.15 \\
        color\_red & 0.09 & 0.53 & 0.15 \\
        color\_saddlebrown & 0.00 & 0.99 & 0.15 \\
        color\_tomato & -0.02 & 0.88 & 0.15 \\
        question\_type\_Determine Range & 0.00 & 0.42 & 0.00 \\
        question\_type\_Find Correlations/Trends & 0.00 & NaN & 0.00 \\
        question\_type\_Make Comparisons & -0.48 & 0.00 & 0.09 \\
        question\_type\_Retrieve Value & -0.74 & 0.00 & 0.09 \\
        \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{Model 3.}
    Regression results.}
    \label{tab:model3_results}
\end{table}


last table together- acc
\begin{table}[htb]
    \centering
    \footnotesize
    \begin{tabular}{lrrrrrr}
        \toprule
        & \multicolumn{2}{c}{\textbf{Model 1}} & \multicolumn{2}{c}{\textbf{Model 2}} & \multicolumn{2}{c}{\textbf{Model 3}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        \textbf{Plot Type} & Coeff. & p & Coeff. & p & Coeff. & p \\
        \midrule
        Pie & -0.04 & 0.57 & -- & -- & -- & -- \\
        Scatter & -0.12 & 0.01 & 0.01 & 0.79 & -- & -- \\
        Bar & -- & -- & -0.02 & 0.65 & -- & -- \\
        Line & -- & -- & -- & -- & 0.65 & ***0.00 \\
        100\% Stacked Bar & -- & -- & -- & -- & 0.17 & †0.07 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Plot type effects across models}.
    Coefficients and p-values shown. 
    Model 1: Uncontrolled; Model 2: Controlled; Model 3: Uncontrolled. 
    *** p < 0.001, † p < 0.1.
    Dashes indicate variable not included.}
    \label{tab:combined_plot_effects}
\end{table}

==> scraps.tex <==

\section{Results}

Here we present our findings on how different visualization characteristics affect MLLM performance.
We organize our results into four key areas: the impact of plot type, the influence of color palettes, the effect of titles, and performance differences when substituting one plot type for another.
For each area, we analyze both accuracy (correct answers) and omission rates (when models chose not to answer) across our expanded VLAT dataset.

\subsection{Impact of Plot Type}

We examined how different visualization types influence MLLM interpretation capabilities through descriptive statistics, statistical tests, and regression analyses.
First, we analyzed accuracy and omission rates across all questions grouped by plot type.
For each question, we tracked (1) the number of correct answers and (2) the number of times the models chose to omit an answer across 20 repetitions, creating performance distributions for each plot type.

% We analyzed the affect of plot type in three stages: first, by examining descriptive statistics, then by conducting statistical tests, and finally by running regression analyses. We start by exploring MLLMs' accuracy and omission rates on all questions, grouped by plot types. We looked at 1) how many questions were correctly answered out of the 20 repetitions, and 2) how many answers were skipped by the model, answering "omit".

We then assigned that question to one of 20 bins, leading to a correctness and a omission histogram for each plot type. Figure \ref{fig:acc_plt_type} shows that some of those performance histograms are quite similar, while others quite different. MLLMs had similar performance distributions when posed with questions based on Line, Scatter and Bar, each question averaging 10.6 to 16 correct counts. The models had proportionally more questions with 20 correct attempts and with 0 omits when answering based on Pie Charts, and had their two worst performances, omission and correctness wise, when responding based on Stacked Bar and its Percentual counterpart.  To complement this analysis Figure \ref{fig:percplot} shows the percentage of questions that were right in every one of the 20 iterations and the percentage of questions that were wrong in every iteration, by plot type. Pie Charts rank the highest with MLLMs responding to 89\% of the questions completely correct while with Stacked Plots, the models managed to respond only 10\% of the questions perfectly. Omission-wise, the same clusters appear: MLLMs omit the most in Stacked Plots, the less on Pie Charts, and an in between amount with Line, Bar and Scatter Plots. 




%percentage of questions with at least 15 correct or something
%from these plots we can get a general sense of the distribution of correct answers and of omits
\begin{figure*}[htbp]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/plot_type_hists2.png}
        \caption{Caption for Figure 1}
        \label{fig:fig1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/omission1.png}
        \caption{Caption for Figure 2}
        \label{fig:fig2}
    \end{subfigure}
    \caption{Overall caption for both figures}
    \label{fig:acc_plt_type}
\end{figure*}
 



\begin{figure}[htbp] % h=here, t=top, b=bottom, p=page
    \centering
    \includegraphics[width=0.5\textwidth]{figures/perc_plot.png} 
    \caption{Omission count distribution over Title Types}
    \label{fig:percplot} % Optional label for referencing
\end{figure}

After this general overview, our next approach was to look into whether different MLLMs had statistically different accuracy and omission when posed with different plot types. After running a Kruskal-Wallis test and finding a very high H-statistic, we confirm that MLLMs had a different accuracy median in at least one of the plot types. In Figure \ref{fig:stat_test} we show a pair-by-pair analysis of model performance in each plot type, showcasing in which of them the model performs significantly different from the other.

\begin{figure}[htbp] % h=here, t=top, b=bottom, p=page
    \centering
    \includegraphics[width=0.5\textwidth]{figures/statistical_test.png} 
    \caption{Median Difference Statistical Test over Title Types}
    \label{fig:stat_test} % Optional label for referencing
\end{figure}
 
 
Values close to 1, represented in blue, show no statistical difference, small values, represented in red, show there is significant statistical difference in model accuracy when grouping these performances by plot type. As seen in the figure, most pairings lead to statistically different medians, and in translation, when not factoring in other elements, it appears as that MLLMs have statistically different accuracies when responding on different plot types. Aligning with the distribution results, when responding based on Line plots, the models do not present statistical difference to responding to Bar or Scatter. Responding to Pie Charts is statistically different than responding to any other plot, and Stacked Bars do not fall under this category only because answering based on them is not statistically different from answering based on their percentual counterpart. 

%today friYAY
%Having drawn from general statistics, and explored statistical tests, we now look over at running different regression models that could further whether plot types affect models' perfomance - even given the presence of other covariates.

%Having drawn from general statistics, and explored statistical tests, we now look over at running the different regression models specified in the Methods section. Those can help us further explore whether plot types affect models' perfomance - even given the presence of other covariates.

Having drawn from general statistics, and explored statistical tests, we now look over at 8 different regression models we ran with the whole dataset. We are particularly interested in the effects of the plot type binary markers because they provide us insight on the relationship between MLLMs' performance and plot types when holding other aspects constant. Table \ref{tab:model_results0} displays results related to model accuracy and Table\ref{tab:model_results} displays coefficient that speak to model omission.

%% NE: This is solely to make the table prettier
\newlength{\minuslength}
\settowidth{\minuslength}{-}
\newcommand{\plus}{\hspace{\minuslength}}

\begin{table}[h]
    \centering
    \rowcolors{2}{White}{SteelBlue!20}    
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lllll}
        \toprule
        \textbf{Question and Plot} & \textbf{Model 1} & \textbf{Model 2} & \textbf{Model 3} & \textbf{Model 4}\\
        \toprule
        plot\_type\_hist & \plus0.54 *** & \plus0.44 *** & -0.14 & \plus0.10 \\
        plot\_type\_line & -0.07 & -0.01 & -0.17 * & -0.13 \\
        plot\_type\_pie & \plus0.89 *** & \plus0.01 & \plus0.31 * & -0.54 *** \\
        plot\_type\_scatter & \plus0.01 & -0.03 & -0.04 & -0.08 \\
        plot\_type\_stacked\_bar & -0.67 *** & -0.59 *** & -0.77 *** & -0.83 *** \\
        plot\_type\_stacked\_bar\_100 & -0.43 & -0.44 *** & -1.19 *** & -1.41 *** \\
        retrieve\_hist &  &  & \plus1.01 *** & \plus1.02 *** \\
        retrieve\_line &  &  & -0.02 & -0.06 \\
        retrieve\_pie &  &  & \plus0.91 *** & \plus0.92 *** \\
        retrieve\_scatter &  &  & \plus0.10 & \plus0.11 \\
        retrieve\_stacked\_bar\_100 &  &  & \plus0.72 *** & \plus0.76 *** \\
        compare\_hist &  &  & \plus0.94 *** & \plus0.96 *** \\
        compare\_line &  &  & \plus0.04 & \plus0.02 \\
        compare\_pie &  &  & \plus0.76 *** & \plus0.77 *** \\
        compare\_scatter &  &  & \plus0.08 & \plus0.11 \\
        compare\_stacked\_bar &  &  & \plus0.28 * & \plus0.26 * \\
        compare\_stacked\_bar\_100 &  &  & \plus1.28 *** & \plus1.32 *** \\
        determine\_range\_line &  &  & \plus0.79 *** & \plus0.62 *** \\
        determine\_range\_scatter &  &  & \plus0.06 & \plus0.00 \\
        \bottomrule
    \end{tabular}%
    }
    \caption{Plot type coefficients accuracy, 3, 2, or 1 stars for significance at 0.1\%, 1\%, and 5\%, respectively. The variables under plot types are interactions between a type of question and a plot type: retrieve is short for value retrieval and compare is short for making comparisons. Model 1 and 3 were not controlled by datasets, Models 2 and 4 were.}
    \label{tab:model_results0}
\end{table}




\begin{table}[h]
    \centering
    \rowcolors{2}{White}{SteelBlue!20}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lllll}
        \toprule
        \textbf{Question and Plot} & \textbf{Model 1} & \textbf{Model 2} & \textbf{Model 3} & \textbf{Model 4} \\
        \toprule
        plot\_type\_hist & -0.04 & -0.08 & -0.09 & -0.11 * \\
        plot\_type\_line & \plus0.07 & \plus0.03 & \plus0.14 ** & \plus0.11 * \\
        plot\_type\_pie & -0.30 *** & -0.02 & -0.26 ** & \plus0.02 \\
        plot\_type\_scatter & \plus0.03 & -0.04 & \plus0.14 ** & \plus0.07 \\
        plot\_type\_stacked\_bar & \plus0.86 *** & \plus1.17 *** & \plus0.84 *** & \plus1.18 *** \\
        plot\_type\_stacked\_bar\_100 & \plus0.61 *** & \plus0.85 *** & \plus0.80 *** & \plus1.15 *** \\
        retrieve\_pie & - & - & -0.16 & -0.19 \\
        retrieve\_scatter & - & - & -0.29 *** & -0.30 *** \\
        retrieve\_stacked\_bar\_100 & - & - & \plus0.63 *** & \plus0.53 *** \\
        compare\_hist & - & - & \plus0.08 & \plus0.11 \\
        compare\_line & - & - & -0.21 ** & -0.17 * \\
        compare\_pie & - & - & -0.74 *** & -0.75 *** \\
        compare\_scatter & - & - & -0.19 ** & -0.17 * \\
        compare\_stacked\_bar & - & - & \plus0.63 *** & \plus0.54 *** \\
        compare\_stacked\_bar\_100 & - & - & -1.20 *** & -1.26 *** \\
        determine\_range\_line & - & - & -0.15 & -0.17 \\
        \bottomrule
    \end{tabular}%
    }
    \caption{Plot type coefficients impact on MLLM omissions, 3,2 or 1 stars for significance at 0.1\%, 1\%, and 5\%, respectively. The variables under plot types are interactions between a type of question and a plot type: retrieve is short for value retrieval and compare is short for making comparisons. Model 1 and 3 were not controlled by datasets, Models 2 and 4 were.}
    \label{tab:model_results}
\end{table}





%plot type regression effects on accuracy
Before we ellaborate on the regression coefficients, we'd like to remind the reader that we are leaving the bar plot binary out so these values are using bar plots as the baseline. 

Having clarified that, the first clear result from the regressions is that plot types are impactful on both MLLM accuracy and on MLLM omission: in 7 of our 8 models, at least 3 different plot types had non-zero significant coefficient and in all our models at least 2 plot types had non-zero significant coefficient. The range of the plot type impact also varies quite a bit. According to Model 4, for example, answering from a Percentual Stacked Plot leads to, on average, a drop in 1.41 standard deviations in the amount of correct questions (in comparison to a Bar Plot). With a standard deviation of around 7.5, that means 10 more wrong answers (out of a total of 20). At the same time, Model 3 shows a decrease of only 0.17 standard deviations (roughly 1 question) in MLLMs' accuracy when responding looking at a Line Plot instead of a Bar Plot.

%these are too much on the 
%The type of impact a specific plot type will have seems to vary less by whether we are measuring impact by accuracy or omission and more by the type of plot itself. Stacked Bar plots and Percentual Stacked Bar Plots, for example, have consistently significant negative coefficients in the accuracy regressions, and consistently positive coefficients when it comes to omissions. In other words, MLLMs seem to get less answers depending on them, and they also seem to omit their answers more. Pie Charts are another example: MLLMs seem to get more answers correctly with them, in comparison to Bar Plots, and omit their answers less. Not a single plot type appeared with the significant effects that had the same signal on omissions and on accuracy.
%On top of the discussed examples, Histograms had somewhat consistent (2 out of 4 models) significant positive coefficients on accuracy and a significant negative coefficient on omissions in 1 model. Line plots appear as a significant negative impact on accuracy, and twice as a significant positive impact on increasing omissions.

Now looking at the interaction variables, the first noticeable thing is how many of them are significant. 8 out of 13 interactions we included in the accuracy models came out as significant, and 7 of them positively. A similar pattern arises in the omissions model, 7 out of 10 interactions are significant, most of them negatively.
When looking at the interactions impact on accuracy, the biggest highlight is the large and positive coefficient for "Making Comparisons" question type with Percentual Stacked Bar. The plot type that came out consistently negatively, when looking at plot types alone, seems to have a rather large (1.32 standard deviations) positive influence on MLLMs accuracy with comparisons-based questions. This is also the only case where a variable that had one sign (i.e. negative) when looking at only plot types had an opposite sign (i.e. positive) in an interaction with a question type. This finding is also consistent with the fact that the Percentual Stacked Bar + Comparison-Based questions combo has a significant negative coefficient on omissions. 
While some interactions also significantly increase accuracy and reduce omissions (Comparison questions and Pie Plots), others increase only accuracy (Retrieval questions and Pie Plots) or only omissions (Comparison Questions and Stacked Bar Plots). But interestingly, Retrieval Questions and Stacked Bar plots is shown to increase both accuracy and omissions, which is also the only interaction that is shown to impact MLLMs in such a way: models tend to get more answers right and at the same time also omit more than when compared to a Bar Plot.

Lastly, we turn to the very model specification to notice that the inclusion of interaction variables (present in Models 3 and 4) did not completely redefine the results we had previously (Models 1 and 2): most of the coefficients maintained significance and their signs. On top of that, the inclusion of datasets underlying the data as a control (Models 2 and 4) did not greatly change the coefficients either, showing consistency of plot types and interaction variables.

%While it is not inconsistent, the behavior raises doubts about the possible causes, which are discussed in the following section of this paper.

 

%Forth, the inclusion of interactions seem to steal some of the results from the plot types, which may happen as they are too correlated with the very occurence of the plot type. This is particularly possible if most questions on a given plot are the interaction we are studying. 



 











%our next approach was to look into the statistics of specific plot transformations. To that end, we aggregated our experiment results by plot transformation, e.g. we grouped by all the answers first answered in a line plot and then answered in a bar plot, and we compared their accuracy.    


%some statistical tests wont hurt
%When looking more precisely, we find that MLLMs had three clusters of performance based on the different plot types. The best cluster was when answering questions related to Histograms and Pie Charts. The models recorded rather high averages and low standard deviations: MLLMs got, on average, 11.8 questions correctly, and had a median of 18 on Histograms. On Pie Chart questions, they had a mean of 18.8 correct questions, a median of 20, and the small standard deviation of 4. The second best cluster of plot types for MLLMs to be asked about were Line, Scatter and Bar plots, where MLLMs had means ranging from 10.6 correct answers on Line Plots to 16 correct answers on Bar plots. Their median on these types of plot varied between 13, 16 and 14, respectivelly. MLLMs had the hardest time answering questions that were posed based on Stacked Bar Plots and Percentual Stacked Bar Plots. The models recorded their lowest mean and median when facing those plots. 
%Now, while model performance revolves mostly around accuracy and reliability, factors tested in the previous statistic, another factor plays an important role, especially given that we are using the VLAT question set as a bechmark: models omissions.


\subsection{Impact of Color Palette}

In order to investigate the possible effects of color palettes on MLLMs performance, we begin by reporting
statistics of how the models performed, accuracy and omission wise, when posed with plots that had different color palettes.
Figure \ref{fig:hist_colors} shows the distribution of questions with different amount of correct answers, broken down by
color palette. The image shows that different color palettes lead to very similar MLLM correctness
performance. The statistics confirm such: the models had an average accuracy that ranged from 10.0 correct 
questions to 10.9. Their medians varied a little more ranging from 10 in the black palette to 14 in the
saddlebrow. Overall, the statistics and the distribution present a very similar picture for model accuracy
irrestrictive of the colors the plot had. This result pattern is maintained when looking at omissions - models 
omitted the most with xxxx, with an average of zzzz and a median of yyyy, and the least with xxxxx.

\begin{figure}[htbp] % h=here, t=top, b=bottom, p=page
    \centering
    \includegraphics[width=0.5\textwidth]{figures/hist_colors.png} 
    \caption{Accuracy distribution through different color palettes}
    \label{fig:hist_colors} % Optional label for referencing
\end{figure}


%Figure \ref{} helps us get a another angle on MLLM omission behaviour between different color schemes, displaying the percentual amount of omited questions per palette. Once again, it is highlighted the high similarity between values.

In light of these conditions, we ran statistical testing to inquiry about whether MLLMs had a statistically different 
accuracy in any of the color palettes. The result of the Kruskal-Wallis test was a rather high p-value of 0.97, and a small H-statistic of 2.84 - the test points in the exact opposite direction of the plot types, indicating that there's no statistical difference towards MLLM accuracy when divided by color palettes. Complementary to that, we ran
the same statistical test for omissions, resulting in a slightly higher H-statistic of 6.54 and a still way too high
p-value of 0.68. This indicates that despite having more variability between them, the diagnosis is the same: MLLMs' 
omission patterns are not statistically different when grouped by different color palettes.


Lastly, we use the different regression models specifications to investigate possible significant coefficient for
the color palette binaries. In none of the 14 different models, with different specifications, we ran, we found any color palette variable to be significant.


\subsection{Impact of Changing the Title}
%this one is still under construction
Lastly, we look at the effect of changing the plot title from a normal title to a suggestive title (that hints at some finding from the visualization). Our results presentation will follow the same structure as of the previous sections. We begin by showing the distribution of questions by the number of correct answers, aggregated by the type of title the plot had, on Figure \ref{fig:histTitle}. 

\begin{figure}[htbp] % h=here, t=top, b=bottom, p=page
    \centering
    \includegraphics[width=0.5\textwidth]{figures/title_hist.png} 
    \caption{Accuracy distribution with different title types}
    \label{fig:histTitle} % Optional label for referencing
\end{figure}

We can see that the two distributions have many similarities. Their means and medians are quite close, despite Normal Titles having a slight advantage, with a median of 12, while Suggestive Titles hold a median of 10. Their most common values for correct responses are 20 and 0, leading both to a bimodal shape, and unlike the previous Chart and Color histograms, they have a much higher percentage of their questions answered completely wrong.

These similarities lead us to perform the same statistical test as we did in the other subsets, Kruskal-Wallis, to verify if MLLMs have statistically different accuracy and omission when answering based on a suggestive-titled plot. The results of the test are a H-statistic of 3.834, and a P-value of exactly 0.05 for accuracy, indicating that MLLMs perform (borderline) statistically differently when handling plots with suggestive titles - though the p-value indicates that this interpretation could go both ways in terms of significancy. When running the same results for omission values, we find a lower H-statistic, at 1.457, and a P-value of 0.227. This indicates (more clearly) that MLLMs' omission is not significantly different when prompted by a plot with suggestive title.

% i need to put the tables
Given the somewhat ambiguous statistical significance observed in the initial comparisons, we turn to regression analysis to further investigate the impact that suggestive titles have on MLLM performance. In all the 8 models we ran, suggestive titles consistently had statistically significant coefficients, always positive on MLLM omission and negative on MLLMs' accuracy. Interestingly, the binary "suggestive\_title" coefficient had the exact same value at two decimal points for all accuracy models, and the same value for all omission models. For the first, the coefficient was -0.06 (standard deviations) and for the latter, -0.07 (standard deviations). In other words, our regression models strongly suggest that MLLMs are very slightly less accurate and very slightly more omissive when Chart Question Answering with a plot that has a suggestive title.

%

\subsection{Evaluating Plot Type Substitution}
%using only plot types that share the same underlying dataset structure
As previously explained, not all plot types in our dataset are logically interchangeable nor comparable due to dimensionality constraints and usability differences. Hence, in order to more clearly investigate the effect of changing from one plot type to the other, we group them into categories where meaningful interchangeability exists. The following groups arise:
\begin{enumerate}
    \item plot types that portray time series-like data (Line, Bar, Scatter)
    \item plot types that portray categorical-based data (Pie Chart, Bar Chart, Scatter)
    \item plots types that portray higher dimensionality categorical-based data (Stacked Bar Plot and Percentual Stacked Bar Plot)
    \item plot types that portray higher dimensionality time series-based data (Stacked Bar Plot, Percentual Stacked Bar Plot, Line)  
\end{enumerate}
 
Within each group, we employ dummy-coded regression to assess how MLLM performance varies across plot types, using a common type as the reference category. This ensures fair comparisons when evaluating how plot type selection impacts MLLM performance. The results are shown in the tables below.



LLM benchmarking is a fundamental part of LLM development as it steers model development in the adequate direction. It can be done in different ways, among which, are the popular ground-truth benchmarks and the more recent LLM-as-judge benchmarks. In the former, LLMs are prompted to respond to a multiple-choice like test, where one answer among the options is correct. In the latter, third-party LLMs are asked to rank the LLMs' answers in an open-ended context. A huge amount of work has been made in LLM benchmarking, spanning a range of different fields from language understanding (references) and overall knowledge (references) to medical attention and sympathy (references), bar exams (references) and of now, there is a somewhat small but growing literature that tackles the LLM data literacy thematic. 

Different authors have elaborated on LLM visualizing capacities of geometric figures and of color, which despite not being data literacy per se, is of direct importance for the field because geometric figures are a fundamental part of data visualizations. Namely, XXXX tested how different LLMs perceive different color palettes. They find that colors like blue and yellow are more easily seen and noticed by LLMs and hypothesize that this comes from their distinctivity. YYYY has found that LLMs have skills in determining the height of 

Extending this line of work and directly tackling the visualization literacy of models are the trailblazing works of Bendeck and Stasko, Li and Hong.
Bendeck and Stasko~\cite{DBLP:journals/tvcg/BendeckS25} and Li et al.~\cite{Li2024} ran different LLMs through the VLAT dataset and summarized their scores on the different types of question VLAT offers, remarking which type of question had a higher score.
Li et al.\ also specifically went on to discuss what could be causing the LLM to fail in some specific tasks. 
%
Hong et al.~\cite{hong25llm} strongly expand the field by having the LLMs respond to each question hundreds of times and by investigating whether the LLMs original training was helping it with the questions. The authors create an alternate version of VLAT without any visual elements that refer to known concepts, as these could aid the LLM go outside the visual scope when answering. 



% \subsection{Our Contributions}

% Our work bases itself on different complementary findings regarding human and MLLM data literacy,  is to craft research that specifies the impact of different visual elements in MLLMs' 



\subsection{Visualization Literacy, Readability, and Assessment}

% Visualization literacy is the ability to read and interpret visual data representations, which is absolutely vital in the information age~\cite{borner_data_2019}. 
% %% Why is visualization literacy is vital?
% With the use of data visualizations becoming popular in news, media, and workplaces, it is essential that users can understand them and derive insights from them. 

% %% How is it measured?
% %% What tests exist
% %% General visualization literacy of people

% %% What is general visualization literacy of LLMs
% %% How do we define visualization literacy in our work?
% %% define visual literacy
% %% define readability
% %% define misleading visualization



% Different authors, despite specific considerations, converge on data visualization literacy being the capability of taking away meaningful information from a visualization. Some highlight the importance of not falling for misconceptions or misleading visual elements, while others elaborate on the user's capability of not only understanding, but also constructing visualizations \cite{ge23}. 

% readability is the property of the plot, but literacy is the ability to read it
% --> how readable the plot is? --> has an impact on the literacy
% \gaby{\cite{cabouat_previs_2024} is on perceived readability}

% Complementary to the works on visualization literacy are long running studies on plot readability.
% Plots consist of smaller visual elements [Grammar of Graphics] and their interplay leads to a logical mapping that helps the user understand what the different visual aspects represent, and how to extend their for meaning [Pinker]. These visual elements are its title, its axes, its colour palettes, and even the type of plot itself. Such internal representations combine with an external context to visually guide the user into the underlying data [Bertin]. Empirically, different authors have found that changing such elements may impact the user perception and takeaways from the visualization. [color paper] finds that using brighter colours damages the user perception, Kong et al. \cite{kong18} found that the title of the visualization heavily impacts what users take away after seeing the plot. 
% \gaby{This is a good moment to introduce our method, like: Inspired by these findings, we conducted a comparative evaluation varying the title, axes, ...}

% Understanding this visual correspondence has become a relevant skill as different fields rely on data visualizations to make crucial decisions. In light of this importance, many authors came up with manners to assess and even numerically evaluate the visualization literacy of a person. One of the most popular assessment frameworks, also present in other LLM benchmark works [references to similar studies], is the Visual Literacy Assessment Test (VLAT) \cite{lee_vlat_2017}. It is a 12-plot, 53-question examination where different aspects of visual literacy are assessed through various question types, such as finding an extremum or commenting on a pattern. Compared to other assessments, VLAT excels at covering diverse visualizations and possible inquiries about them. It also provides an easy-to-use, openly available dataset containing all questions, question types, and underlying visualization data. 
% VLAT focuses on the human side of the evaluation, but literacy also befalls on the plot. As different studies point out directly or indirectly, the elements of the plot heavily matter to how easy it is to be consumed.


% It is important, however, to highlight that while these theoretical and empirical works converge in interesting findings, they were made based on the human cognitive system, and when exposing a data visualization to an LLM, that will consume it rather differently, new findings emerge, as shown in Sect. \ref{sec:llmliteracy}. While VLAT and other examinations might suffice for quantitative analysis of human individuals, assessing LLMs require larger samples that can lead to statistically significant results.

%results from an in-depth comparative evaluation of GPT-4o and Gemini Pro 2.0 for an expanded VLAT test focusing on reliability, generalized charts, and context; 
%(2) a set of visualization design principles that facilitates both human and LLM visualization literacy; and


% %% How LLMS understand data visualizations
% %% Why do we need LLMs literacy?: for BLV users? or could it be more general? or maybe say that we don't know of all the potential use cases
% %% Use cases: automatic pattern detection: for outliers, anomaly detection, etc
% Large Language Models (LLMs) have been one of the biggest topics in academia and industry, and stemming from their popularity and possible benefits is a wide array of benchmark research. These investigate how well these models perform human-dominated tasks like code generation, math exercises, IQ tests and even bar exams and medical diagnostics. Despite this growing research, many fields where LLMs could have, or are already having, a direct impact remain overlooked in the LLM benchmark world, data visualization understanding and literacy being one of the clearest examples. Because a lot of written material LLMs excel at summarizing or consulting include data visualizations, a lot of tech that portrays visualizations to blind or visually impaired people rely on LLMs now and for better general understanding of LLM vision, we need to better understand whether and how these models understand data visualizations.

%% What is our contribution?
%% dataset based on VLAT: which is "unique" in terms of titles, plot types, color palettes

% To better assess LLM's capacity in the data visualization world, we create an unique dataset based on the classic VLAT dataset \cite{lee_vlat_2017}, but extended with new titles, new color palettes and new plot types for each of the original visualizations. By repeating the original questions to all visualizations that come from the same data, we leap from 12 original plots to 380 plots, and from a 60-row dataset to a 1380 one. We then have two different LLMs, Google Gemini and ChatGPT 4.0, go through the plots and answer each related question. Given LLMs known stochastic aspect, however, we decided to ran each VLAT question 20 times, and instead of just relying on one answer, we used the pass@k metric to better represent really how well the model does. 

% By expanding the original dataset more than 30 times, and running each question 20 times, we hope to achieve a much more consistent assessment of how different visual aspects impact LLMs' data literacy. This variety of data points with controlled changes helps us single out different visual elements' impact on LLM understanding and the sheer size of both the data and the repetition of our assessment helps us understand whether this type of assessment was trustworthy in the first place: not only what affects the LLM response but also, if this effect lasted multiple iterations. To summarise, we attempt to answer three main research questions:

% Previous works study the extent to which LLMs have visualization literacy \cite{hong25llm}, and what are their limitations. In contrast, our work focuses on aspects of visualization that impact LLM visual literacy and can we design rules for improving LLM visualization literacy.
% RQ1. Which visual aspects like plot type, color palette and title are associated with better LLM performances?
% RQ2. How reliable are LLMs' responses concerning their data literacy? 
% RQ3. What are, and are there, design rules for better visualization literacy for an LLM


% In summary, we continue to push the benchmark for LLMs on data visualization by expanding the usual modelling scenario and, perhaps most importantly, incorporating a fundamental aspect of LLMs into the problem: their stochasticity. 

% % We generate important findings around which aspects of the visualization seem to matter the most in these models' understanding of visualizations: we find that some specific types of question matter, the title seems to matter quite a bit, and none of the "types" of visualization seem to matter a lot. We also find which of these aspects make the model less trustworthy, that is, with which of those the model scrambles and has a higher variance in their responses. Both of these, not seen in previous literature. Lastly, we make both the code and the dataset available for further research to explore it. 

